Hypercube drawings with no long plane paths

We study the existence of plane substructures in drawings of the $d$-dimensional hypercube graph $Q_d$. We construct drawings of $Q_d$ which contain no plane subgraph with more than $2d-2$ edges, no plane path with more than $2d-3$ edges, and no plane matching of size more than $2d-4$. On the other hand, we prove that every rectilinear drawing of $Q_d$ with vertices in convex position contains a plane path of length $d$ (if $d$ is odd) or $d-1$ (if $d$ is even). We also prove that if a graph $G$ is a plane subgraph of every drawing of $Q_d$ for a sufficiently large $d$, then $G$ is necessarily a forest of caterpillars. Lastly, we give a short proof of a generalization of a result by Alpert et al. [Cong. Numerantium, 2009] on the maximum rectilinear crossing number of $Q_d$.

==> Obsoletemaybe/miscellaneous.tex <==
\begin{theorem}
Let $k\in \mathbb{N}$ and $G=(E,V)$ be a graph with $|V|=n$ and $E\ge kn$. Then, any convex-geometric drawing of $G$ contains a plane path of length at least $2\lfloor \frac{k-1}{2} \rfloor+1$.  
\end{theorem}

\begin{proof}
Let $\Gamma$ be a convex-geometric drawing of $G$. We construct a sequence of convex-geometric drawings $\Gamma_0,
\Gamma_1,\Gamma_2,\dots, \Gamma_{\lfloor\frac{k-1}{2}\rfloor}$ of subgraphs of $G$ in the following way.  We start with  $\Gamma_0 = \Gamma$. Then, we obtain $\Gamma_1$ from $\Gamma_0$ by removing the leftmost edge adjacent to each vertex.  Then, for $i\in\{2,\dots, \lfloor\frac{k-1}{2}\rfloor\}$ we obtain $\Gamma_i$ alternatingly removing the rightmost and leftmost edge at every vertex. It is clear by our assumptions that $\Gamma_{\lfloor \frac{k-1}{2} \rfloor}$ contains at least one edge $e=uv$. In the following we assume that $\lfloor\frac{k-1}{2}\rfloor$ is odd and therefore $\Gamma_{\lfloor\frac{k-1}{2}\rfloor}$ was obtained from $\Gamma_{\lfloor\frac{k-1}{2}\rfloor-1}$ by removing the leftmost edge at every vertex. But since $e$ was not removed from $\Gamma_{\lfloor\frac{k-1}{2}\rfloor -1}$, it was not the leftmost edge of any of its endpoints. Let $l_u=uu'$ and $l_v=vv'$ be the leftmost edges of $u$ and $v$ respectively. Then, $l_u,e$ and $l_v$ together form a plane path with three edges. Now, since $l_u$ and $l_v$ were not removed from $\Gamma_{\lfloor\frac{k-1}{2}\rfloor}-1$, it means that $l_u$ and $l_v$ were not the rightmost edges of $u'$ and $v'$ and we can again find two edges that extend this path. Since we can repeat this argument $\lfloor\frac{k-1}{2}\rfloor$, in the end we obtain a path consisting of $2\lfloor\frac{k-1}{2}\rfloor+1$ edges.
\end{proof}

We obtain the following result about hypercubes as an immediate corollary. 

\begin{corollary}
Any convex-geometric drawing of $H_d$ contains a plane path of length at least $d-3$.
\end{corollary}


\section{Stuff about length profiles}
All possible length profiles for 4-hypercube (probably not complete, sorry):
\begin{enumerate}
    \item 1,2,2,6
    \item 1,2,3,5
    \item 1,2,3,7
    \item 1,2,4,4
    \item 1,2,4,6
    \item 1,2,4,7
    \item 1,2,4,8
    \item 1,2,5,7
    \item 1,2,6,6
    \item 1,3,5,6
    \item 1,3,6,7
    \item 1,4,4,6
    \item 1,4,6,8
    \item 1,5,6,7
    \item 2,2,5,6
    \item 2,3,4,4
    \item 2,3,4,5
    \item 2,3,4,8
    \item 2,3,6,7
    \item 2,4,4,5
    \item 2,4,4,7
    \item 2,4,5,8
    \item 2,4,6,7
    \item 2,4,7,8
    \item 2,5,6,6
    \item 3,4,4,6
    \item 3,4,6,8
    \item 4,4,5,6
    \item 4,4,6,7 (our rotation of square)
    \item 4,5,6,8
    \item 4,6,7,8 (our rotation of hour glass)
\end{enumerate}



In a length regular graph:
\begin{enumerate}
\item There must be at least one odd length otherwise the graph is not connected.

\item If there are two odd lengths $l_{i}, l_{j}$ then either $l_{i}+l_{j}$ or $l_{i}-l_{j}$ cannot exist. This is because each odd length up to symmetry has one scenario. We get two scenarios for the combinations of $l_{i}$ and $l_{j}$, in one $l_{i}+l_{j}$ creates a triangle and in the other one $l_{i}-l_{j}$. So one of them is forbidden.
\begin{itemize}
    \item For the forbidden one also its multiples are forbidden since it will lead to an odd cycle.
    \item Especially the diagonal is forbidden.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=.6\linewidth]{odd scenarios.jpg}
    \caption{The two scenarios for a combination of length 3 (pink) and 5 (green) in 4-hypercube. Left: length $5-3=2$ (both scenarios) creates a triangle; right: length $5+3=8$ creates a triangle.}
    \label{fig:placeholder}
\end{figure}
    \item  If a length appears twice, no even multiple of it can appear; otherwise, it would generate an odd cycle.



    \item If an odd number appears twice, no even number can appear, as there is an even path from $0$ to any even point, so the existence of that edge would create an odd cycle.  



    \item Every pair of odd lengths blocks one even length and its multiples. The diagonal is a multiple of every edge.

    \item With respect to odd edges, there are only two rotation vectors and they alternate around the circle.
\end{enumerate}

\begin{conjecture}
    \begin{enumerate}
        \item For lengths $\ell_1\leq \ell_2\leq ...$ we have $l_i\leq 2^{d-1}-2^{d-(i+1)}$.
        \item There have to exist edges of even length (for $d\geq 4$?, for $d$ even?)
        \item If length $\ell$ is odd, it cannot occur twice (for $d\geq 3(4)$). 
    \end{enumerate}
\end{conjecture}




==> TIKZ_files/tikzcommands.tex <==
\newcommand{\RotationalCoordinates}[1]{
	%\coordinate (Z) at (0,0);
    \pgfmathsetmacro{\nsquare}{2^#1}
	\foreach \i in {-\nsquare,...,\nsquare}{
		\coordinate (R\i) at (360/#1*\i:2);
	}
	%\foreach \i in {0,...,#1}{
	%	\pgfmathparse{mod(int(1+\i),#1)}
	%	\pgfmathsetmacro{\nxt}{\pgfmathresult}
	%	\coordinate (S\i) at ($(R\i)+(R\nxt)$);
	%}
}

\newcommand{\circulararcgraph}[2]{
    \pgfmathsetmacro{\d}{#1}
     \pgfmathsetmacro{\n}{2^\d}
     \RotationalCoordinates{\n}
%     \draw (R1) -- (R2) -- (R3);
    \foreach \k in {#2} {
            \foreach \v in {1,...,\n}
                \pgfmathsetmacro{\w}{\v+\k}
                \draw (R\v)--(R\w);
        }

}


\newcommand{\Lengthregulardrawing}[3]{% dimension, lengths that are double (incl diagonals), lengths that are once
   \pgfmathsetmacro{\d}{#1}
    \pgfmathsetmacro{\n}{2^\d}
    \RotationalCoordinates{\n}
    \foreach \k in {#2} {
            \foreach \v in {1,...,\n} {
                \pgfmathsetmacro{\w}{\v+\k}
                \draw (R\v)--(R\w);
            }
    }
    \foreach \l in {#3} {
        \pgfmathsetmacro{\a}{\l[1]}%length   - 2
        \pgfmathsetmacro{\twoa}{\a*2}%twicethelengthlength - 4
        \pgfmathsetmacro{\exponentvector}{\l[2]}%length - {1}
        \pgfmathsetmacro{\g}{\gcd(\a,\n)} % 2^nr of cicles - 2
        \pgfmathsetmacro{\ng}{log2(\g)} % nr of circles - 1
        \pgfmathsetmacro{\h}{\n:\ng} %length of circle
            \foreach \c in {0,...,\ng-1} {%which circle
                \foreach \i in {1,..,\h:2}{%where in the circle
                    \pgfmathsetmacro{\firstvertex}{\c+\i*\twoa}
                    \pgfmathsetmacro{\exponent}{\exponentvector[\c]}
                    \pgfmathsetmacro{\sign}{(-1)^\exponent}
                    \pgfmathsetmacro{\difference}{\sign*\a}
                    \pgfmathsetmacro{\secondvertex}{\firstvertex+\difference}
                    \draw (R\firstvertex)--(R\secondvertex);
                } 
            }
    }
    

        
%        \foreach \i in #3 {%length
%               \pgfmathsetmacro{\l}{\gcd(2^#1,\i)}
%               \foreach \j in {1,...,\l} {
                    
%               }
%        }

}

\newcommand{\Lengthregulardrawingone}[3]{% dimension, lengths that are double (incl diagonals), lengths that are once, #one choice
   \pgfmathsetmacro{\d}{#1}
    \pgfmathsetmacro{\n}{2^\d}
    \RotationalCoordinates{\n}
    \foreach \k in {#2} {
            \foreach \v in {1,...,\n} {
                \pgfmathsetmacro{\w}{\v+\k}
                \draw (R\v)--(R\w);
            }
    }
     \foreach \l in {#3} {
            \foreach \r in {1,...,\n} {
                \pgfmathsetmacro{\firstvertex}{\l*\r*2}
                \pgfmathsetmacro{\s}{\firstvertex+\l}
                \draw (R\firstvertex)--(R\s);
            }
    }
}    

    
%    \foreach \l in {#3} {
%        \pgfmathsetmacro{\a}{\l}%length   - 2
%     %   \pgfmathsetmacro{\twoa}{\a*2}%twicethelengthlength - 4
%        \pgfmathsetmacro{\h}{\n} %length of circle
%                \foreach \i in {1,..,\h}{%where in the circle
%                    \pgfmathsetmacro{\firstvertex}{\i}
%                    \pgfmathsetmacro{\difference}{\a}
%                    \pgfmathsetmacro{\secondvertex}{\firstvertex+\difference}
%                    \draw (R\firstvertex)--(R\secondvertex);
%                } 
%            
%    }
%}
    



